The Global Magneto-Ionic Medium Survey (GMIMS): The brightest polarized region in the Southern sky at 75cm and its implications for Radio Loop II

Using the Global Magneto-Ionic Medium Survey (GMIMS) Low-Band South (LBS) southern sky polarization survey, covering 300 to 480 MHz at 81 arcmin resolution, we reveal the brightest region in the Southern polarized sky at these frequencies. The region, G150-50, covers nearly 20deg$^2$, near (l,b)~(150 deg,-50 deg). Using GMIMS-LBS and complementary data at higher frequencies (~0.6--30 GHz), we apply Faraday tomography and Stokes QU-fitting techniques. We find that the magnetic field associated with G150-50 is both coherent and primarily in the plane of the sky, and indications that the region is associated with Radio Loop II. The Faraday depth spectra across G150-50 are broad and contain a large-scale spatial gradient. We model the magnetic field in the region as an expanding shell, and we can reproduce both the observed Faraday rotation and the synchrotron emission in the GMIMS-LBS band. Using QU-fitting, we find that the Faraday spectra are produced by several Faraday dispersive sources along the line-of-sight. Alternatively, polarization horizon effects that we cannot model are adding complexity to the high-frequency polarized spectra. The magnetic field structure of Loop II dominates a large fraction of the sky, and studies of the large-scale polarized sky will need to account for this object. Studies of G150-50 with high angular resolution could mitigate polarization horizon effects, and clarify the nature of G150-50.

==> abstract.tex <==
The Global Magneto-Ionic Medium Survey (GMIMS) has, for the first time, imaged the entire Southern sky in linear polarization at low radio frequencies with full spatial sampling and broad bandwidth. This survey, GMIMS Low-Band South (LBS), covering 300 to 480 MHz, has revealed the brightest region in the Southern polarized sky at these frequencies. The region, G150$-$50, covers nearly 20\,$\deg^2$, near ${l,b}{\approx}{(150^{\circ}},-50^{\circ})$. Using GMIMS-LBS and complementary data at higher frequencies, we apply Faraday tomography and Stokes $QU$-fitting techniques to analyse G150$-$50. We find that the magnetic field associated with G150$-$50 is both coherent and primarily in the plane of the sky, and indications that the region is associated with Radio Loop II. The Faraday depth spectra across G150$-$50 are broad and contain a large-scale spatial gradient. We model the magnetic field in the region as an expanding shell, and we can reproduce both the observed Faraday rotation and the synchrotron emission in the GMIMS-LBS band. Using $QU$-fitting, we find that the Faraday spectra are produced by several Faraday dispersive sources along the line of sight. Alternatively, polarization horizon effects that we cannot model are adding complexity to the high-frequency polarized spectra. The magnetic field structure of Loop II dominates a large fraction of the sky, and studies of the large-scale polarized sky will need to account for this object. Studies of G150-50 with high angular resolution could mitigate polarization horizon effects, and clarify the nature of G150$-$50.

